Selective Weak Supervision for Neural Information Retrieval

This paper democratizes neural information retrieval to scenarios where large scale relevance training signals are not available. We revisit the classic IR intuition that anchor-document relations approximate query-document relevance and propose a reinforcement weak supervision selection method, ReInfoSelect, which learns to select anchor-document pairs that best weakly supervise the neural ranker (action), using the ranking performance on a handful of relevance labels as the reward. Iteratively, for a batch of anchor-document pairs, ReInfoSelect back propagates the gradients through the neural ranker, gathers its NDCG reward, and optimizes the data selection network using policy gradients, until the neural ranker's performance peaks on target relevance metrics (convergence). In our experiments on three TREC benchmarks, neural rankers trained by ReInfoSelect, with only publicly available anchor data, significantly outperform feature-based learning to rank methods and match the effectiveness of neural rankers trained with private commercial search logs. Our analyses show that ReInfoSelect effectively selects weak supervision signals based on the stage of the neural ranker training, and intuitively picks anchor-document pairs similar to query-document pairs.

==> Archive/eva.tex <==
\section{Evaluation Results}
Six experiments are conducted to evaluate \ris{}'s effectiveness. We also provide human evaluations and case studies on the selected weak supervision data.
% This section shows the overall results on the two benchmark datasets, effectiveness of policy network, REINFORCE data selection, data strategies and fine-tuning strategies. The case studies are also conducted.

\subsection{Overall Results}
This part presents the overall results of \ris{} and all baselines, as shown in Table~\ref{tab:overall}. Two neural ranking models, Conv-KNRM and BERT are our main baselines. Three trained strategies with unannotated data are compared: \texttt{Anchor+BM25 Labels}~\cite{dehghani2017neural}, \texttt{Title Discriminator}~\cite{macavaney2019content} and \texttt{All Anchor}. The \texttt{Title Discriminator} utilizes trained neural ranking models, such as Conv-KNRM, to classify title-document pairs for the week supervision training data. \texttt{Anchor+BM25 Labels} and \texttt{All Anchor} are two strategies to select anchor-document pairs with the BM25 based ranking score and random sample.

For Conv-KNRM, \ris{} significantly outperforms the \texttt{No Weak Supervision} model, which indicates the anchor corpus plays an important role for training neural ranking models. \ris{} also outperforms trained neural ranking models, \texttt{Title Discriminator} \texttt{Anchor+BM25 Labels} and \texttt{All Anchor}, significantly. The better performance illustrates the effectiveness of data selection with reinforcement learning and rewards from environment can guide a better data selection policy. Moreover, \ris{} outperforms \texttt{Anchor+BM25 Labels} by large margins, which demonstrates the advance of week supervision between anchor text and linked documents for neural ranker training.

The BERT ranker is trained with document-level corpus and the anchor based training also helps for a significant improvement, which demonstrates the anchor based training is more concentrated on query and document ranking than language model. In addition, the \ris{} shares almost the same performance with \texttt{Bing User Clicks} trained neural ranking models~\cite{dai2019deeper}. The available anchor corpus shows its advance for neural ranker training and provides an opportunity to improve the general ranking performance for information retrieval. 

The overall results present the effectiveness of \ris{} for training neural ranking models. However, it is still unclear what brings such improvement to neural rankings and the following experiments explore the source of neural ranker's improvement.

\subsection{Effectiveness of Policy Network}
\input{Tables/policy.tex}
This part explores the effectiveness of policy network.
The performance of three kinds of state, \texttt{A State} ($s^a$), \texttt{A-D State}  ($s^{ad}$) and \texttt{All State} ($s$) are presented in Table~\ref{tab:policy:state}.

The overall classification accuracy of ClueWeb09-B is less than Robust04. For the classifier, it is harder to classify queries of ClueWeb09-B than queires in Robust04 from the anchor and query set. The queries from ClueWeb09-B are more like the anchor text. For ClueWeb09-B, \texttt{All State} presents the best performance than others for anchor-document classification, which illustrates the effectiveness of \texttt{All State} for anchor and query classification.

For Robust04, \texttt{A State} shows the lowest query classification accuracy among all state representations, while \texttt{A-D State} performs the best classification score. The interactions between the query (or anchor) and relevance document  help to distinguish real queries and help to achieve better classification score. However, the \texttt{A-D State} filter lots of query-like anchors and these misleading anchors usually contain important supervised signals for training neural ranking models. \texttt{All State} is the trade-off of real query classification and the number of pseudo training instances.

The \texttt{All State} presents convinced classification accuracy on different datasets and shows its effectiveness on data selection. The next part further explores the performance of different state representations and different data selection methods.



\subsection{Effectiveness of REINFORCE data selection}
\input{Figures/reinforce.tex}
This part explores the effectiveness of REINFORCE data selection with different strategies, as shown in Table~\ref{tab:policy:class}. \texttt{A Discriminator}, \texttt{A-D Discriminator} and \texttt{All Discriminator} represent the pipeline of two steps: classify anchor-document pairs that like real queries from all anchor corpus and then train the neural ranker with selected anchor data. The rest results are from \ris{}. \texttt{Scratch} and \texttt{Warm Up} indicate if the data classifier is pre-trained with the supervision from anchor and query discriminator.

All data selection methods outperform the \texttt{ALL Anchor}, which illustrates the anchor data is informative but noisy and the data selection is necessary to filer query-like data from anchors. Then the reinforce based data selection methods outperform all pipeline models, which further demonstrates the effectiveness of \ris{}.
\texttt{All state} shows better performance than other state representations, which illustrates \texttt{All state} can better select query-document pairs and include enough anchors, even though some pairs can be distinguished to `fake'. The \texttt{All state} satisfies the underlying information need by selection anchor instances for neural ranking model during training. Moreover, the pre-trained data classifier (\texttt{Warm Up}) is more effective than the no-trained data classifier (\texttt{Scratch}). The supervision from query and anchor discriminator is an important prior signal for the data selection. Nevertheless, the no-trained data selection (\texttt{Scratch}) also can reach a comparable performance with the pre-trained data classifier (\texttt{Warm Up}).

The \ris{} shows convinced performance for training neural ranking models and provides a potential way to select data to satisfy the underlying information need for neural ranking models during training. The next part will explore the effectiveness of different data strategies.

\input{Figures/datastrategy.tex}
\input{Tables/finetune.tex}
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.24\linewidth]{Pictures/action_c.png} \includegraphics[width=0.24\linewidth]{Pictures/reward_c.png}
	\caption{Action and Reward.
	\label{fig:training}}
\end{figure*}


\subsection{Effectiveness of Data Strategies}

This part presents the effectiveness of data strategies.
Different numbers (10K, 50K, 100K and 500K) of the higher ranking score anchors are selected according to the \texttt{All State} classifier and the performance is presented, as shown in Table~\ref{tab:data}.

The performance of neural ranker is increased and becomes the peak with 100k anchors, while add more anchors (500k) the model performance is decreased dramatically. This phenomenon illustrates that the anchor corpus is noisy and the noisy anchors will mislead neural ranking models to a worse performance. To fit the general neural ranking scenario, for a anchor, the linked documents are treated as weak positive documents and the negative documents are sampled according to the score from unsupervised retrieval models, such as BM25. To further explore the effectiveness of different data strategies, we utilize 100k anchors and include different ratios of positive documents and negative documents, 5:6, 3:7 and 2:8. The total training pairs of different ratios are kept almost same. The 5:6 ratio based data strategy performs much better than 3:7 and 2:8, which demonstrates the more weak positive documents are included the more improvement is achieved. The weak relevance of anchor text and document is the most crucial part for \ris{} and is more useful than the BM25 scores based weak supervision.



This part presents different performance of different data strategies of \ris{} because the anchor data is noisy. The week supervision from the relevance between the anchor text and its linked documents is more effective than BM25 scores based weak supervision. The next part will explore the effectiveness of different fine-tuning strategies for ranking features from different models for the further improvement.

\subsection{Fine-Tuning Strategies}

This part explore the effectiveness of ranking features from three models: unsupervised retrieval model \texttt{SDM} and two neural ranking models, \texttt{Conv-KNRM} and \texttt{BERT}. The the performance from different learning to ranking (LeToR) strategies are compared. All results are presented in Table~\ref{tab:finetune}.

For different learning to ranking strategies, the \texttt{Coor-Ascent} outperforms \texttt{Dense Layer} by a large margin, which demonstrates the effectiveness of feature based learning to ranking methods and \texttt{Coor-Ascent} can better aggregate ranking features. Then the traditional ranking feature (\texttt{SDM}) and additional neural ranking features (\texttt{BERT}) are added to features from Conv-KNRM step by step. The ranking performance is increased while more features are added, which indicates different models learn ranking features from different aspects and all features contribute to a better ranking performance. The \texttt{Discriminator} and \ris{} presents the different training strategies for neural models. The experimental results from \ris{} all outperform the results from \texttt{Discriminator}, which further demonstrates the \ris{} can better satisfy the underlying information need of neural ranking models than the pipeline based data selection strategy. The consistent improvement illustrates the robustness and effectiveness of \ris{}.

The studies on different fine-tuning strategies show the feature based learning to ranking methods better aggregate ranking features for further improvement. The \ris{} also illustrate the effectiveness with different learning to rank scenarios. The next part will present the action and reward state of \ris{} during stochastic training to further explore the effectiveness of \ris{}.


\subsection{Stochastic Training}
In this part, the stochastic training process of \ris{} is presented in Figure~\ref{fig:training}. The average action score and reward are performed, which indicate the data selection ration and the environment reward, respectively.

For both average action score and reward, the score of the two training scenarios, \texttt{Warm Up} and \texttt{Scratch}, tend to the same value with the growth of training step. Nevertheless, at the beginning of training, \texttt{Warm Up} shows less instance selection and more reward than  \texttt{Scratch}. It is distinctly that pre-trained data selection select more query-like anchors for training of neural rankers. The average data selection ratio of \texttt{Warm Up} is increased dramatically and decreased with the increasing of training step because of the immature neural ranker. It is necessary for data selector to provide training data according to the need of neural ranker instead of the classification ability of anchor-query classification. Both the data selector and neural ranker promote each other for the further improvement. 

The average action score and reward performance during training process present \ris{} feed training instances according to the training state of neural ranker. Only well-trained anchor-query classification is not enough to satisfy the neural ranker with different training states.



\subsection{Selected Weak Supervision Pairs}
\input{Figures/agreement.tex}

\cx{A Table of Discriminator, Conv-KNRM \ris{} and BERT \ris{} agreements, and number of selected/not selected pairs}

\cx{A human evaluation results of anchor selection accuracy and anchor-document relation accuracy as  the preferred document vs negative in human evaluation}


\subsection{Case Study}
This part describes the case study.

Selected queries, and queries that hurts

The documents selected and discarded for the selected queries.

\input{Tables/case.tex}











==> Archive/intro.tex <==
\section{Introduction}



Recently, neural models have proven their effectiveness in ad-hoc retrieval. Training the neural ranking models require large-scale supervised data, which consists of the query that real human asked and documents they clicked. However, the data is usually kept as commercial secret by search engine company, and is not open to the public. To address this problem, we view anchor text in web pages as pseudo query, and the texts they link as documents. The links are viewed as a weak supervised signal that the pseudo query and documents are relative. There is much noisy data in the pseudo query and documents, such as fake relevance. These noise data may damage NRMs' performances.

There are many possible ways to prevent performance damages caused by noise data. Training a heuristic-based or discriminator filter to select the pseudo query and documents. The filters learn to classify the supervised and weak supervised data. Thus, the selected data are similar to the supervised data. Another method is learning a reinforced agent rewarded by the performance of target model, which in this work is a NRM, to select high-qualified data. The reinforced method first selecting pseudo data, training the target model on them, and evaluating performance of the pre-trained NRM on benchmark datasets.

This work proposes a framework that integrating a reinforced data selector into NRMs. Given a set of pseudo query and its relevant document pairs, our framework first selects a subset of high-quality data by the data selector, which is learned directly from the reward of NRM's performance. We follow the actor-critic algorithm for the data selector agent, the policy chooses an action whether remove a sample or not based on the state of it. The representation of state is the crucial for data selection. We proposed a new state that include the representations of query, document and query-document interaction. The query and document representations are from CNN and self-attention, query-document interaction are pooling by kernels.

We experiment our pre-trained NRMs on two ad-hoc retrieval benchmark datasets: ClueWeb09-B and Robust04. The performances of our NRMs trained on weak supervised data are competitive to that of NRMs trained on user logs in search engine. Our experiments demonstrate that the reinforced data selector...

In the rest of this paper, Section 2 discusses related work, Section 3 presents our reinforced data selector for filtering weak supervised data to pre-train NRMs framework, Experimental methodology and evaluation results are described in Section 4 and 5, Section 6 is about the conclusions and future work.

==> Archive/related.tex <==
\section{Related Work}
Neural ranking models (NRMs) can be divided into two categories: representation based models and interaction based~\cite{guo2016matching}. Representation based models learn low-dimension representations of query and documents, and calculate the relevance score for ranking. DSSM~\cite{jiafeng2016deep} and CDSSM~\cite{cdssm} are two typical representation based models. They utilize word hashing to get word representations and a shallow neural network is leveraged for the query and document representations. Interaction based models learn word-level interactions between query and documents for the ranking score. MatchPyramind~\cite{Pang2016TextMA} uses Convolutional Neural Network (CNN) to encode interactions between query and documents to get ranking features. K-NRM~\cite{xiong2017knrm} and Conv-KNRM~\cite{convknrm} model query and document interactions with long-desired exact and soft match patterns which provides a variety of relevance match signals with Gaussian kernels. Some models~\cite{www2017duet} further combine the interaction based and representation based methods for improvements.

Pre-trained models ,such as ELMO~\cite{} ,provide an
%Training NRM to reach good performance requires a large amount of supervised data, such as user query logs. Recently, pre-trained models have developed rapidly. The Conv-KNRM adapted by Bing search log was the previous state-of-the-art neural Ranking model. Google's BERT is trained on large-scale corpus by masked language model and self attention, and has advanced the state-of-the-art on many NLP tasks, even including information retrieval tasks. Dai et al. augments BERT with Bing log, further benefits BERT effectiveness on ad-hoc retrieval.

However, the search log data is usually not accessible for the public. Utilizing weak supervised data is one way to address this problem. Some early works use anchor texts or news titles as pseudo query. Recently, Dehghani et al. uses the AOL query log and produce documents by BM25 results as weak supervised signal that the top ranked documents are more relevant to the query. MacAvaney et al. argues that BM25 has its limits that the top ranked documents are not necessarily more relevant to the query, and uses news headline and its content as relevant text pair, further proposes k-max filter, which calculates MSE on interaction matrices, then selects k training samples most close to the target data.

To select high-quality source domain training data, distance function, GAN, RL...

Reinforced Data Selector takes the performance growth of the transferrable model in target domain as a reward to learn to select better source domain data for model pre-training. Reinforcement learning (RL) has been widely used not only in the Atari games, but a variety of deep learning tasks. RL can be roughly divided into two categories: value based and policy based. The value based methods estimate future expected total rewards through a state, such as deep Q network. Policy based methods try to directly find the next best action in the current state, such as REINFORCE algorithm. To reduce variance, some methods combine value based and policy based methods for more stable training, such as the actor-critic algorithm. There are already some methods for data selection based on RL. However, there is a lack of reinforced data selection methods to solve search tasks.

Sentence representation...
